Confidence from Invariance to Image Transformations

We develop a technique for automatically detecting the classification errors of a pre-trained visual classifier. Our method is agnostic to the form of the classifier, requiring access only to classifier responses to a set of inputs. We train a parametric binary classifier (error/correct) on a representation derived from a set of classifier responses generated from multiple copies of the same input, each subject to a different natural image transformation. Thus, we establish a measure of confidence in classifier's decision by analyzing the invariance of its decision under various transformations. In experiments with multiple data sets (STL-10,CIFAR-100,ImageNet) and classifiers, we demonstrate new state of the art for the error detection task. In addition, we apply our technique to novelty detection scenarios, where we also demonstrate state of the art results.

==> Figures/manipulated_images_fig.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{Figures/manipulated_images.png}
	
	\caption{\label{fig:manipulated_images}\textbf{Correctly and incorrectly classified STL10 images. }From left to right: The original images, their manipulated versions and their corresponding (color-coded) soft-max outputs (obtained using the pre-trained classifier of \cite{DistBasedScore_Mendelbaum2017}). While both images obtain the same confidence score according to the SR method (red dashed line), the soft-max values of the misclassified (upper) image fluctuate across manipulated versions, while those of the correctly classified (lower) image are relatively stable.}
	{\vspace{-0.2cm}}
\end{figure}


==> Tables/error_detect_detector_types.tex <==
\begin{table}[!tbh]
	\begin{center}
		\begin{tabular}{|c||c|c|c|c|c|c|}
%			\hline
%			\multirow{2}{*}{}& \multicolumn{3}{c}{STL-10} & \multicolumn{3}{|c|}{CIFAR-100}\\\cline{2-7}
%			& Regular & Dist. & AT & Regular & Dist. & AT\\
%			\hline
%			Baseline \cite{Baseline_Hendrycks2016} &&&&&&\\
%			\cite{DistBasedScore_Mendelbaum2017} &-&-&-&-&-&-\\
%			\cite{Dropout_Gal2015} &&&&&&\\
%			Ours &&&&&&\\
%			\hline
		\end{tabular}
		\vspace{5pt}
	\caption{\label{tab:error_detect_detector_types}\textbf{Error detection using different detectors.}}
	\end{center}
\end{table}


==> Tables/error_detect_my_classifiers_table.tex <==
\begin{table}[!thb]
	\begin{center}
		\begin{tabular}{|c||c|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{}& \multicolumn{3}{c}{STL-10} & \multicolumn{3}{|c|}{CIFAR-100}\\\cline{2-7}
			& Regular & Dist. & AT & Regular & Dist. & AT\\
			\hline
			Baseline \cite{Baseline_Hendrycks2016} &&&&&&\\
			\cite{DistBasedScore_Mendelbaum2017} &-&-&-&-&-&-\\
			\cite{Dropout_Gal2015} &&&&&&\\
			Ours &&&&&&\\
			\hline
		\end{tabular}
		\vspace{5pt}
		\caption{\label{tab:error_datect_methods_our_clsfr}\textbf{Error detection performance on our pre-trained classifiers.} AUROCC of our method (bottom row) vs. the baseline method\cite{Baseline_Hendrycks2016}, the method of Mendelbaum and Weinshall \cite{DistBasedScore_Mendelbaum2017} and MC-Dropout \cite{Dropout_Gal2015}, when tested on classifiers trained by \cite{DistBasedScore_Mendelbaum2017}}
	\end{center}
\end{table}


==> Tables/error_detect_transformations.tex <==
\begin{table}[!t]
	\begin{center}
		\begin{tabular}{|c||c||c|c|c|c|c||c|}
			\hline
%			Using STL-10_Amit_AT classifier, with detectorTrain. Blur:52
			% \hhline{-||-----}
			\diagbox[innerwidth=2.9cm,trim=r]{Detector}
%			{Manipulation}& Original&(1) Flip & (2) Gamma & (3) Contrast & (4) Blur & (5) BW & ALL\\
			{Manipulation}& Original&Flip & Gamma & Contrast &Blur & Gray scale & ALL\\

			\hline
%			MSR \cite{Baseline_Hendrycks2016}&0.807/0.888&-&-&-&-&-&-\\
%			KL divergence&-&0.809/0.893&0.787/0.886&0.798/0.888&0.797/0.89&0.708/0.834&-\\
%			MLP&0.813/0.892&&&&&&0.851/0.906\\
			MSR \cite{Baseline_Hendrycks2016}&0.807&-&-&-&-&-&-\\
			Ours, KL divergence&-&0.809&0.787&0.798&0.797&0.708&-\\
			Ours, MLP&0.813&0.834&0.821&0.824&0.825&0.822&0.846\\
			\hline
		\end{tabular}
	\vspace{5pt}
	\caption{\label{tab:error_detect_transformations}\textbf{Error
            detection using different image transformations, STL-10}
          AUROC values of detectors based on scores of different image
          transformations. First row values correspond to directly
          using the KL-divergence score, while second row values are
          obtained using MLP on top of the logits. All detectors are applied on the \emph{Regular} classifier of \cite{DistBasedScore_Mendelbaum2017}. }
%	 (*Baseline NN operates on the logits of original images)
	\end{center}
\end{table}

